New Properties and Invariants of Harmonic Polygons

Via simulation, we discover and prove curious new Euclidean properties and invariants of the Poncelet family of harmonic polygons.

==> 090_video_table.tex <==
Animations illustrating some invariant phenomena herein are listed on Table~\ref{tab:playlist}.

\begin{table}[H]
\small
\begin{tabular}{|c|c|l|l|}
\hline
id & N & Title & \textbf{youtu.be/<.>}\\
\hline
01 & 5 & {Invariants of $\F$} &
\href{https://youtu.be/2PdsC3CcqaE}{\texttt{2PdsC3CcqaE}}\\
02 & 3 & {Invariant Brocard Angles over $F$ 3-gons} & \href{https://youtu.be/2fvGd8wioZY}{\texttt{2fvGd8wioZY}} \\
03 & 3 & {Locus of Brocard Points $\F$ 3-gons} & \href{https://youtu.be/13i3JGY-fK4}{\texttt{13i3JGY-fK4}}\\
04 & 5 & {Invariant signed area of Evolute Polygon, $s=\{.25,.5,.75,.1\}$} & \href{https://youtu.be/JCj0q7_hlA8}{\texttt{JCj0q7\_hlA8}} \\
05 & 3,5,6,8 & {Evolute Polygons with Zero Signed Area} & \href{https://youtu.be/3nvXYFoI5Wg}{\texttt{3nvXYFoI5Wg}} \\
06 & 5 & {Invariant-Area Evolute Polygon with $s=1$} & \href{https://youtu.be/ChsfLzKrb4o}{\texttt{ChsfLzKrb4o}} \\
07 & 3 & {Zero-area Evolute Polygon is a horizontal segment} & \href{https://youtu.be/f80QaYs5_J4}{\texttt{f80QaYs5\_J4}} \\
08 & 3 & {Two zero-area evolute polygons intersect on $X_{76}$} & \href{https://youtu.be/OFA_j25R8ks}{\texttt{OFA\_j25R8ks}} \\
\hline
\end{tabular}
\caption{Illustrative videos. The last column is clickable and provides the YouTube code.}
\label{tab:playlist}
\end{table}



==> 210_app_symbols.tex <==
\begin{table}
\small
\begin{tabular}{|c|l|l|}
\hline
symbol & meaning & note \\
\hline
$\E,\E_c$ & outer and inner homothetic ellipses & \\
$N$ & vertices of $N$-gon & \\
$O$ & center of concentric pair & \\
$a,b$ & semi-axes of $\E$ & \\
$c$ & half the focal length of $\E$ & $c^2=a^2-b^2$ \\
$a_c,b_c$ & semi-axes of $\E_c$ & $(a_c,b_c) = \cos(\pi/N) (a,b)$ \\
$P_i,\theta_i$ & Poncelet vertices and angles & $i=1,...,N$\\
$f_1,f_2$ & foci of $\E$ & $[\pm c,0]$ \\
$d_{j,i}$ & distance from $P_i$ to $f_j$ & $|P_i-f_j|$ \\
$s_i$ & $i$-th sidelength & $|P_{i+1}-P_i|$, $i+1$ mod $N$\\
$A,L$ & area and perimeter & $\sum{s_i}$ \\
$L_{2}$ & sum of squared sidelengths & $\sum{s_i^2}$ \\
$\omega$ & Brocard angle ($N=3$) & $\cot\omega=L_{2}/(4A)=\sum\cot{\theta_i}$ \\
$\mathcal{P}_s,\ell_i$ & evolute polygon and its $i$-th sidelength & \\
\hline
\end{tabular}
\caption{Symbols used.}
\label{tab:symbols}
\end{table}


==> 999_refcheck.tex <==
\usepackage{refcheck}
% make refcheck work w cref
% https://tex.stackexchange.com/questions/87610/making-refcheck-work-with-cleveref
\makeatletter
\newcommand{\refcheckize}[1]{%
  \expandafter\let\csname @@\string#1\endcsname#1%
  \expandafter\DeclareRobustCommand\csname relax\string#1\endcsname[1]{%
    \csname @@\string#1\endcsname{##1}\@for\@temp:=##1\do{\wrtusdrf{\@temp}\wrtusdrf{{\@temp}}}}%
  \expandafter\let\expandafter#1\csname relax\string#1\endcsname
}
\newcommand{\refcheckizetwo}[1]{%
  \expandafter\let\csname @@\string#1\endcsname#1%
  \expandafter\DeclareRobustCommand\csname relax\string#1\endcsname[2]{%
    \csname @@\string#1\endcsname{##1}{##2}\wrtusdrf{##1}\wrtusdrf{{##1}}\wrtusdrf{##2}\wrtusdrf{{##2}}}%
  \expandafter\let\expandafter#1\csname relax\string#1\endcsname
}
\makeatother

\refcheckize{\cref}
\refcheckize{\Cref}
\refcheckizetwo{\crefrange}
\refcheckizetwo{\Crefrange}

==> ender.tex <==
\vskip .5cm
\noindent Dan Reznik, \texttt{dreznik@gmail.com} \\ 
 Data Science Consulting\\
Rio de Janeiro, RJ, Brazil, 22210-080
 

